GASKAP Pilot Survey Science II: ASKAP Zoom Observations of Galactic 21-cm Absorption

Using the Australian Square Kilometre Array Pathfinder to measure 21-cm absorption spectra toward continuum background sources, we study the cool phase of the neutral atomic gas in the far outer disk, and in the inner Galaxy near the end of the Galactic bar at longitude 340 degrees. In the inner Galaxy the cool atomic gas has a smaller scale height than in the solar neighborhood, similar to the molecular gas and the superthin stellar population in the bar. In the outer Galaxy the cool atomic gas is mixed with the warm, neutral medium, with the cool fraction staying roughly constant with Galactic radius. The mean spin temperature, i.e. the ratio of the emission brightness temperature to the absorption, is roughly constant for velocities corresponding to Galactic radius greater than about twice the solar circle radius. The ratio has a value of about 300 K, but this does not correspond to a physical temperature in the gas. If the gas causing the absorption has kinetic temperature of about 100 K, as in the solar neighborhood, then the value 300 K indicates that the fraction of the gas mass in this phase is one-third of the total HI mass.

==> Gau_fits_inc_2ph_22oct.tex <==
%\hspace{.02in}\raisebox{2cm}{\includegraphics[width=3.6in]{Termv_1panel_22oct21_incl_Gal.pdf}
% updated 8 sept for wtmin=25, n=150  now 22 oct 21 wtmin=25 n=148 
%\FloatBarrier
%\startlongtable
%\begin{deluxetable}{|l|l|l|l|l|l|l|l|}
%\tablecaption{Gaussian Fits to the Absorption vs. Latitude near the Terminal Velocity
%\label{tab:Gaussians}}
%\tablehead{\colhead{velocity range} &
%\colhead{peak} & \colhead{b center} & \colhead{$\sigma{b}$ width} & \colhead{T${_s}$} & \colhead{peak}& \colhead{b center} & \colhead{$\sigma_b$b width}} \\ 
%\colhead{km s$^{-1}$} &
%\colhead{$1-e^{-\tau}$} & \colhead{(deg)} & \colhead{(deg)} & \colhead{(K)} &
%\colhead{$1-e^{-\tau}$} & \colhead{(deg)} & \colhead{(deg)}}\\
%
\begin{table} \caption{Gaussian Fits to Absorption vs. Latitude near the Terminal Velocity \label{tab:Gaussians}}
%\hspace{-2cm}\begin{tabular}{|l|lll|l|lll|}
\hspace{-2cm}\begin{tabular}{|c|ccc|c|ccc|}
\hline
 & \multicolumn{3}{c|}{weighted fit}& & \multicolumn{3}{c|}{unweighted fit}\\
velocity range & $\tau$ peak & b center & $\sigma_b$ width &  T$_{s}$ & $\tau$ peak & b center & $\sigma_b$ width  \\
km s$^{-1}$ &$1-e^{-\tau}$ & deg & deg & K & $1-e^{-\tau}$ & deg & deg \\ \hline
%\startdata
-145 $< v <$ -125 & 0.30$\pm$0.02 & 0.0$\pm$0.04 & 0.59$\pm$0.03  &   & 0.29$\pm$0.02 & +0.03$\pm$0.05 & 0.62$\pm$0.04 \\
\hline
-125 $<v<$ -100 & 0.27$\pm$0.02 & -0.05$\pm$0.03 & 0.51$\pm$0.03 &    & 0.28$\pm$0.02 & -0.05$\pm$0.04 & 0.58$\pm$0.04 \\
\hline
-100 $<v<$ -75  & 0.40$\pm$0.02 & +0.07$\pm$0.02 & 0.50$\pm$0.02 &    & 0.36$\pm$0.02 & +0.04$\pm$0.03 & 0.58$\pm$0.03  \\
\hline  
-135 $<v<$ -100 & 0.29$\pm$0.01 & -0.07$\pm$0.03 & 0.60$\pm$0.02 &  160 & 0.30$\pm$0.01 & -0.04$\pm$0.03 & 0.61$\pm$0.03  \\
\hline  
0 $<v<$ +8 & 0.37$\pm$0.03 & +0.11$\pm$0.05 & 0.59$\pm$0.05  & 123 & 0.37$\pm$0.03 & +0.08$\pm$0.05 & 0.47$\pm$0.06\\
$\tau$ baseline & 0.34$\pm$0.02 &&&&  0.37$\pm$0.02&&\\
\hline 
+15 $<v<$ +30 & 0.39$\pm$0.02 & -0.62$\pm$0.03& 0.60$\pm$0.03 & 176 & 0.42$\pm$0.02 & -0.76$\pm$0.03 & 0.63$\pm$0.04 \\
\hline
+45 $<v<$+65 &0.05$\pm$0.01 & -0.27$\pm$0.052 & 1.20$\pm$0.06 & 325 & 0.05$\pm$0.01 & -0.15$\pm$0.20 & 1.43$\pm$0.25\\
\hline
\hline
\multicolumn{8}{|c|} {Two Phase Emission Fit} \\
\hline
& \multicolumn{3}{c|}{CNM} & T$_{CNM}$ & \multicolumn{3}{c|}{WNM}\\
-135 $<v<$ -100 & 35 K & -0.074 & 0.596 & 121 K & 11 K & +0.1 & 1.6 \\ 
\hline
\end{tabular}
\end{table}


